A Low-Cost, Controllable and Interpretable Task-Oriented Chatbot: With Real-World After-Sale Services as Example

Though widely used in industry, traditional task-oriented dialogue systems suffer from three bottlenecks: (i) difficult ontology construction (e.g., intents and slots); (ii) poor controllability and interpretability; (iii) annotation-hungry. In this paper, we propose to represent utterance with a simpler concept named Dialogue Action, upon which we construct a tree-structured TaskFlow and further build task-oriented chatbot with TaskFlow as core component. A framework is presented to automatically construct TaskFlow from large-scale dialogues and deploy online. Our experiments on real-world after-sale customer services show TaskFlow can satisfy the major needs, as well as reduce the developer burden effectively.

==> introduction.tex <==
\section{Introduction}

% 食品安全问题是个challenge—>发现食品安全相关的事件能够缓解这个challenge—>尽管事件检测已经well researched，但是limited work在做这个工作，原因在于缺少食品安全相关的数据集。

% 食品安全问题是个challenge—>发现食品安全相关的事件能够缓解这个challenge
Nowadays, food safety remains a grand challenge to human health, especially in developing countries \cite{lv2018engineering,fung2018food,qin2021soil}. 
Detecting food safety events can not only discover the risky food providers or restaurants, but also release early warnings for consumers, thus considered to have the potential to effectively alleviate such challenge.

Event detection (ED), which aims to identify event triggers and classify them into specific types from unstructured texts, has been widely researched and applied in various downstream tasks.
The advanced models have been continuously proposed, including the feature-based models \cite{liao:2010using,hong-etal-2011-using,li2013joint} and neural-based models \cite{chen2015event,nguyen2016joint,yan-etal-2019-event,chen-etal-2018-collective,zheng2019doc2edag,wang2020maven,xie-etal-2021-event,xiangyu-etal-2021-capturing}. 
Though achieving significant progress, few efforts have been devoted to food safety event detection. One possible reason is the lack of benchmarking datasets, which play an important role in enabling the development and evaluation of ED models for food safety.
% 现有的数据集主要集中在了general domain，例如ACE 2005、MAVEN等；
Most existing works exploits general domain benchmarks (e.g., ACE 2005 \cite{walker2006ace}, TAC KBP datasets \cite{mitamura2015overview} and MAVEN \cite{wang2020maven}) and focus on the common events in people's life, such as ``being born'', ``getting married'', ``being arrested'', ``divorce'', etc. 
% 同时有一些垂直领域的数据集，例如blabla；但是并没有针对食品安全进行研究的数据集
Some datasets are proposed recently to facilitate the exploration in specific domains. For example, \cite{zheng2019doc2edag} builds the ChFinAnn dataset with Chinese financial announcements, which contains five typical finalcial event types.
\cite{satyapanich2020casie} and \cite{trong2020introducing} build the CASIE and CySecED datasets, which annotates the articles on websites and mainly cover cybersecurity events such as ``Root Compromise'' and ``Denial of Service''.
However, none of existing datasets contain food safety events and can be served as benchmarks.

% Our observation shows that food delivery apps很受欢迎—>用户在上面留下了大量的交互信息，例如评论/售后客服/电话客服等，为发现食品安全事件提供了可能性。如果能够及时从这些UGC中发现食品安全相关的事件，就能够做到预警，并及时发现食品存在问题的食物提供者。

Our observation is that with the rapid development of e-commerce, online food service platform are more popular, and people increasingly select restaurants and order food through food delivery apps such as Doordash\footnote{https://www.doordash.com/} and Meituan\footnote{https://meituan.com}. Also, app users tend to give feedbacks on food safety issues in different ways, such as posting reviews and communicating with after-sale staffs. 
Such user behaviors generate large scale and timely data which contains valuable information about food safety events and can serve as benchmarks.

% 本文做了什么
% 1. 数据选择从Meituan的多个源头进行了提取
% 2. 从用户、骑手和商家三个角度定义了food safety events schema
% 3. 标注了大规模的数据集
To this end, we present a human-annotated massive food safety event detection dataset (named FoodSafetyED), for the first time. FoodSafetyED has the following characteristic:
\begin{enumerate}
    \item \textbf{Multi-domain} We collect and desensitize data from three typical scenarios of Meituan, which is China's leading e-commerce platform for food services:
i) user post reviews about specific order; ii) user communicate with after-sale staff online through text messages; iii) user communicate with after-sale staff through telephone. Thus, the corpus consists of user reviews, text conversations and telephone conversations.
    \item \textbf{Broad Coverage} From users' perspective, we construct a food safety event schema, which contains 21 event types and cover users' in-depth descriptions of food, restaurant, delivery person, and their own physical feelings. 
    \item \textbf{Large scale} The FoodSafetyED dataset contains 11,381 documents, 315473 sentences and 36,883 event mentions. In terms of instance number per event type, FoodSafetyED outperform other datasets with a large margin (i.e., 1756 of FoodSafetyED v.s. 707 of MAVEN v.s. 104 of ACE 2005 v.s. ).
\end{enumerate}
% Specifically, we collect and desensitize data from three typical scenarios of Meituan \footnote{https://meituan.com}, which is China's leading e-commerce platform for food services:
% i) user post reviews about specific order; ii) user communicate with after-sale staff online through text messages; iii) user communicate with after-sale staff through telephone.
% Furthermore, we construct a food safety event schema from users' perspective, which contains 21 event types and cover users' in-depth descriptions of food, restaurant, delivery person, and their own physical feelings. 
% Finally, through human annotation, we construct the large scale FoodSafetyED, which contains 11,381 documents, 313,616 sentences and 36,883 event mentions.

\begin{figure}[h]

\centering
\includegraphics[scale=0.4]{example.pdf}
\caption{Instances from \textit{text conversations}, \textit{telephone conversations} and \textit{user reviews} in FS-CMED.}
\label{fig:data}
\end{figure}

% 对实验进行概括，说明challenge

% 总结main contribution
Our contributions can be summarized as follows:
\begin{enumerate}
    \item To facilitate investigation of food safety event detection, we present a large scale dataset, named FoodSafetyED, for the first time.
    \item As pioneer research, we present strong baselines and valuable exploration, which can inspire broader investigation in the future.
\end{enumerate}


% through after-sale customer services. 









